PSPC: Efficient Parallel Shortest Path Counting on Large-Scale Graphs

In modern graph analytics, the shortest path is a fundamental concept. Numerous \rrev{recent works} concentrate mostly on the distance of these shortest paths. Nevertheless, in the era of betweenness analysis, the counting of the shortest path between $s$ and $t$ is equally crucial. \rrev{It} is \rev{also} an important issue in the area of graph databases. In recent years, several studies have been conducted in an effort to tackle such issues. Nonetheless, the present technique faces a considerable barrier to parallel due to the dependencies in the index construction stage, hence limiting its application possibilities and wasting the potential hardware performance. To address this problem, we provide a parallel shortest path counting method that could avoid these dependencies and obtain approximately linear index time speedup as the number of threads increases. Our empirical evaluations verify the efficiency and effectiveness.

==> directed.tex <==
\section{Extension to Directed Graphs}
\label{sec:direct}
For a weighted directed graph $G = (V, E,l(\cdot))$, where $l(e) > 0$ signifies the weight of an edge $e$, instead of $L_{\leq}(v)$, two labels $L^{in}_{\leq}(v)$ and $L^{out}_{\leq}(v)$ are calculated for each vertex $v$. Specifically, a vertex $w$ that satisfies $w \leq v$ is chosen as a hub in $L^{in}_{\leq}(v)$ (resp. $L^{out}_{\leq}(v)$ ) if and only if there exists at least one trough shortest path from $w$ to $v$ (resp. from $v$ to $w$). To compute $L^{in}_{\leq}(·)$, in HP-SPC, Dijkstra’s algorithm instead of BFS is performed from each vertex in the forward direction. Afterward, Dijkstra’s algorithm is executed again in the backward direction to calculate $L^{out}_{\leq}(\cdot)$. A query $(s, t)$ is evaluated by scanning $L^{out}_{\leq}(s)$ and $L^{in}_{\leq}(t)$.


Before using 1-shell reduction, we first calculate the 1-shell of $G$ as if $G$ is undirected. Afterward, for each linked component $cc$ (in the undirected sense) of the 1-shell, we construct a reachability oracle for $cc$ $\cup$ $a(cc)$. For any vertices $u,v \in cc \cup a(cc),$ let reach$(u,v) = 1$ if $v$ is reachable from $u$ in $G$ and $= 0$ otherwise. Consider a query $(s,t)$. If $s$ and $t$ come from the same $cc$, the $\#$ of shortest paths from $s$ to $t$, $spc(s,t)$, is exactly reach$(s,t)$; otherwise, $spc(s,t)$ $=$ $reach(s, shr(s))$ $\cdot$ $spc(shr(s), shr(t))$ $\cdot$ $reach(shr(t),t)$. 
Regarding weighted directed graphs, we redefine neighborhood equivalence as follows. Let $nbr_{in}(v)$ and $nbr_{out}(v)$ be the in-neighbors and out-neighbors of a vertex $v$, respectively.

==> limitations.tex <==
\section{Limitations of this work}
\label{sect:limit}

We discuss some limitations of this work in the following.

\noindent \textbf{Maintenance under Dynamic Updates}. Given a graph $G$, a labeling $L(\cdot)$ for $G$ and an update $\Delta G$ to $G$, the problem of dynamic labeling under $\Delta G$ is to maintain $L(\cdot)$ such that the resulting labeling is the corresponding one for $G \oplus \Delta G$, where $G \oplus \Delta G$ is the graph obtained by applying $\Delta G$ to $G$. For canonical distance labeling, the existing dynamic algorithms all fail to achieve high efficiency while retaining the minimality of the labeling~\cite{akiba2014dynamic,akiba2012shortest,qin2017efficient}, and it is still an open problem regarding how to address this issue. Since our labeling $L \leq (\cdot)$ contains the canonical labeling $L^c_{\leq}(\cdot)$ as a subset, the same challenge persists when designing a dynamic algorithm for $L^c_{\leq}(\cdot)$. Worse yet, the necessity to maintain the information about $\sigma_{v, w}$ can further complicate the design.


\noindent \textbf{Indexing Size}.~As shown in the experiments, although we could speed up the indexing time by increasing the number of threads. Nevertheless, for some graphs such as DB and FL, our algorithms require far more index space than other graphs of similar size. Unfortunately, thus far it is still not clear what properties of these graphs lead to this inefficiency. Is there an efficiently computable ordering that effectively handles these graphs? Or is the huge resource consumption inevitable even with an optimal ordering under the current
labeling scheme? Both of the questions are also open.


==> tech2.tex <==
\section{Optimizations}
\label{sect:tech2}
This section introduces some optimization techniques to further speed up our algorithm.


\subsection{Landmark-Based Filtering}
\label{subsect:land_prune}
This subsection introduces landmark pruning. Landmark-based techniques are proved to be efficient in the Label Constrained Reachability problem~\cite{valstar2017landmark}. The overall idea is to select some small sets of vertices as landmarks and construct some small indexes on them to speed up the whole index construction process. It follows their strategies to select landmarks. To begin, this part introduces the definition of landmarks.
\begin{definition}
\label{def:land}
(Landmark).~
Given a threshold $\theta$, a vertex $v$ is a landmark if and only if $degree(v) \geq \theta$.
\end{definition}

In the index construction process, the distances from landmarks are frequently used. Based on this observation, this work proposes landmark-based filtering to further speedup the index construction process. 

In the classical shortest path counting with a 2-hop labeling index, vertices are explored individually. It processes vertex serially. For a vertex $u$, once it is explored, there is no need to utilize its distance information due to the pruning rule 1. Thus, there is no need to construct such a landmark index. 

Nevertheless, the facts change for our parallel algorithm. As for the parallel algorithm, the label propagation is divided by distance round. Thus, in each round, the labels from the landmarks would be the majority since the degree of the landmarks are very large. Thus, if the distance information is stored from these landmarks, these queries could be immediately answered if landmarks are involved.

Furthermore, since all the distances are in the increasing order. It is necessary to need one bit to store the ``True'' or ``False'' information, and it is sufficient to answer queries for pruning.


